OmniStyle: Filtering High Quality Style Transfer Data at Scale

In this paper, we introduce OmniStyle-1M, a large-scale paired style transfer dataset comprising over one million content-style-stylized image triplets across 1,000 diverse style categories, each enhanced with textual descriptions and instruction prompts. We show that OmniStyle-1M can not only enable efficient and scalable of style transfer models through supervised training but also facilitate precise control over target stylization. Especially, to ensure the quality of the dataset, we introduce OmniFilter, a comprehensive style transfer quality assessment framework, which filters high-quality triplets based on content preservation, style consistency, and aesthetic appeal. Building upon this foundation, we propose OmniStyle, a framework based on the Diffusion Transformer (DiT) architecture designed for high-quality and efficient style transfer. This framework supports both instruction-guided and image-guided style transfer, generating high resolution outputs with exceptional detail. Extensive qualitative and quantitative evaluations demonstrate OmniStyle's superior performance compared to existing approaches, highlighting its efficiency and versatility. OmniStyle-1M and its accompanying methodologies provide a significant contribution to advancing high-quality style transfer, offering a valuable resource for the research community.

==> 1000_style.tex <==
100 years, 11, Vogue magazine cover illustrations in 1920-1930, Mavis cosmetics and perfume advertisements in the 1920s, 2.5D1, 2.5D2, 2.5D3, 2.5D4, 2.5D5, 2.5D6, 2.5D creative illustration subject gradient color, 2.5D isometric charm architecture, 2.5D urban life and social relations, 2.5D style house commercial illustration, 3D1, 3D2, 3D3, 3D4, 3D avant-garde character modeling and color matching fashion and technology, 3D modeling exquisite details trend art, 3D comics, 3D stereo UIICON, 3D stereo modeling design geometric graphics, 3D style, 8  16  24 pixel style 2, 8  16  24 pixel style 3, 90s TV games, Abigail J Harding's dark fairy tale, AdamGustavson thick painting, AdamastorStudio, Aki, AlessandraScandella, AliceinWonderland, AndrewArcher plane perspective, AnnaRudak, Antoine Corbineau color graffiti stitching fashion, Audreyhelenweber1, Blockprint style illustration, BrianGallagher black and white, C4D Monster MONSTER, C4D abstract art high-end color matching, CASTLESINAIRS, CG computer graphics, COSMO Beauty September virtual environment The beauty of truth, Caver black cat illustration with fresh and natural colors and texture, ChiaraMorra vector, ChrisBianchi black and white, Christian Gralingen's graphic illustration poster, Christine Anderson, Cindy SalansRosenheim, DamienJeon black and white, DanlinZhang, Daria, Dave Plunkert pink and black, Desdichas de una family victor, Dream boats and other stories, DuairakPadungvichean, Dustoftime, EduFuentes paper-cut style, EmmaZanelli European and American style realism, EricPautz, Eveline Tarunadjaja decorative line, Flower Fairies of the Spring, GeorgeBarbier, Georges Lepape American retro fashion illustration, GoncaloViana, HENNKIM, Hamlet surreal beauty, HieuHoang, HouseGarden magazine cover, Imagine a city picture book, Isabel Klett Children's Picture Book, JUNde Immersive Diary Visual Modeling, Joanna Grodecka, Jocelin Carmes, Jolo's Bizarre Adventure, Jonathan Rice, Juan Bernabeu, Justin Wood Synthesis, KIMBERLEY WISEMAN, Katewong, Katherine Bradford, Kezia Gabriella, Kristina Vasiljeva Realism, LOWPOLY, Laurie Hastings Fresh Flat, Laurie Greasley American, Leegan Koo, Linda Carruth, Lomo style photo 1, Lomo style photo 2, Lucy Truman black and white sketch, Luis Pinto vision, MBE style, MELANIE GANDYRA, MET flat clay freeze, MONICALind, Mam BA, Marc Mones children's illustration, Mark Samuel watercolor, MarkGregory American Realism, MarkMatcho American Comics, MattDartfordAJMDIDigital3D, MelcherOosteman, MelcherOosteman Interesting Visual Illustration, MichaelMeister, MonicaKamakura, NFT, NOTITEL, Nabil Nezzar, NancyRose, Nathan Rohlander Realism, NathanRohlander Realism American, NathanSmith3D, Nick Hayes Color Stereotype, Nick Hayes Black and White Stereotype, OliverBurston Synthetic Medical, Olivia Knapp Black and White Decorative Painting Realism, PILYEON, PILYEON Black and White, PacoPomet, RWDS, RokasAleliunas, SelectedWorks, Spaceflower, SummerLien, SusanLugar, TINA, The boy who kewn what the birds said, TheWillowTreeFae, Tina Guan Qier Blue and White Porcelain Pattern Print Scene Illustration, Tobias kwan Destiny 2 Partial Concept Design, ToniDemuro, TravisFoster, TreeofSavior, Unity Creative Style, VansFaces, VeraPavlova, VickiHerring Decoration, WakanaYamazaki, Welder Wings Hyperrealistic Gothic, Will Bradley Book and Poster Print Illustration, YURERU, Youneedpotato Hand-painted, YurikoShirou, ZHOU Color matching is fresh and elegant  the composition is simple and highlights the subject, adelina lirius, andre ducci, ashiyaart, b18art, carlo quaranta, carlod 2, city pop, climatechangeaffects, culturefestivalEvent, deadprince, deco, Donapp Small Reunion Commercial Illustration, ellice weaver, eune rvu, feitufei1, feitufei2, feitufei3, feitufei5, feitufei6, feitufeiuivi1, gastaus sketches, guyen elegant and ethereal, happy geometric illustrations, havana illustrations 2, hawaiiansalad, ipad modeling white film carving meticulously, jessprintdesigns, k2, kathrin honesta, kristinvestgard, magicpockets visual composition, marcello velho, memoryspaceofsol Korean style, minimalist, nanaco yashiro, noelle fantasy planet, ofraamit picture book style, ori toor, peacock marker graffiti fashion, pocky mini, reoenl two-dimensional, ronald kuang, stevesimpson, sungmooheo original painting, tameimpala visual composition, ullathynell, vergilho, vintagecard, watercolorillustration, yinakim, yvecz fairy tale, z22742624 ultra-detailed stereotyped scene, A strange and fantastic sea adventure at first sight, Magic illustration Joshua Raphael, Original illustration of the cycle of life and death, All things picture book, Kaleidoscope-like illustrations of the twelve zodiac signs, Long vacation in the 1930s retro travel poster, 3D rendering 2, Original IP image story of 3D rendering, Sleeping Beauty picture book of the last century, Shanghai Film Animation Studio, Different daily corners of life, Different work  different office areas  European and American style, World famous Agatha book cover, Tokyo Olympic picture book illustrations  exaggerated dynamic characters  rich colors, Tokyo Story series posters  two-dimensional anime style, The subtlety of oriental blank space and the ingenious fusion of western minimalist concepts, Oriental beauties are drawn with lines as the skeleton, Oriental aesthetics  ancient style  exquisite and gorgeous details, Oriental aesthetics has no logic but order, Oriental poetry and painting 1, Oriental poetry and painting 2, Medieval classical style  western clothing  animal forest illustrations, Collection of illustrations of Chinese myths and legends, Exquisite and textured illustrations of ancient Chinese myths, Monochrome illustrations of medieval picture books, Nature elements of Chinese traditional culture Dunhuang series, Chinese paper-cutting art  German version, Chinese ancient fine brushwork flower and bird paintings by Yu Jigao, Chinese Strange Tales Illustrations Guo Zikai sheep, China Daily New National Trend Creative Illustrations, Chinese Folk Tales Legends Nine Songs, Chinese Folk Tales Seizing the Pearl and Eliminating the Pests Picture Book, Chinese Style Scene Illustrations Grand and Magnificent, Chinese Style Aesthetics Sija Hong Six Li 1, Chinese Style Aesthetics Sija Hong Six Li 3, Chinese Style Aesthetics Sija Hong Six Li 4, Chinese Style Aesthetics Sija Hong Six Li 5, Chinese Style Aesthetics Sija Hong Six Li 6, Chinese Style Aesthetics Sija Hong Six Li 7, Chinese Style Aesthetics Twenty-four Solar Terms Ancient Style Illustrations, Chinese Style Aesthetics Ni Chuanjing 1, Chinese style aesthetic Ni Chuanjing 2, Chinese style aesthetic Si Ye eating fish, Chinese style aesthetic illustration Mian Lang 1, Chinese style aesthetic illustration Mian Lang 2, Chinese style aesthetic illustration Mian Lang 3, Chinese style aesthetic illustration Mian Lang 4, Chinese style aesthetic painter Ibuki Chicken Leg, Chinese style aesthetic painter Shan Ze, Chinese style aesthetic painting Yu Yuqing, Chinese style aesthetic Lu Mingshan 1, Chinese style aesthetic Lu Mingshan 2, Chinese style element guide page, Chinese style painting style, The lines of Chinese freehand brushwork comic strips are decorative, The rich imagination and complex content and colors have a strong impact, The rich painting elements and symmetrical composition form are full of details, Rural style 1, Rural style 2, Book page art, Random line painting in the picture comic woodcut illustration, 2D, 2D 2, 2D original painting 1, 2D original painting 2, 2D original painting 3, 2D original painting 5, 2D illustration 1, 2D illustration 2, 2D illustration 3, 2D illustration style, Yunnan Dai folk legend illustration, Colorful future world trend commercial illustration, Yanai Jasmine 1, King Arthur illustration woodcut, 19 years of skeletonization of the dead, People and fantasy creatures, Rich flat insertion of portrait silhouettes, Combination of characters and plant images, Life is a fairy tale written by the hand of God, Painting with blocks of color to retain the texture of the brushstrokes, Yiyaer's Chinese style line drawing, Beautiful lines outline the softness of the characters, Traditional and modern combined  East and West collide, Traditional Chinese ink painting style 1, Traditional Chinese ink painting style 2, Traditional culture 1, Traditional culture 2, Traditional Japanese aesthetics  street culture  colorful comic style, Traditional crayon photo filter, Vulgar noir style, Low polygon 2, Low poly style 2, Russian fairy tale illustration style is unique and rich, Russian lines have strong contrast and epic scenes, Playful life illustrations, Seurat, Comic strips borrowed from Dunhuang murals, Ni Chuanjing, Flat vector illustration charity project, Flat style commercial illustration of the same color, Nuo opera mask, Children's illustration dopamine milk tea shop, Children's 2.5D, Children's illustrator Ana Sanfelippo, Children's illustrator Nina dzyvulska, Children's illustrator choomoranma, Children's illustrator oimoeee, Children's illustrator rongart, Children's illustrator seulart, Children's illustrator Anastasia, Children's illustrations are extremely simple lines and low-saturation colors, Children's illustration Paidomi creates growth fragments, Children's illustrations are funny and humorous, Children's watercolor illustrations, Children's healing picture book with exquisite details, Children's picture book Balbuzar's adventure story, Children's picture book with complex black and white lines, Children's picture book onion is humorous and interesting, Children's picture book uses bold colors with slightly clumsy brushstrokes, Children's picture book with exquisite details  warm colors  warm and healing, Children's picture book style gray tone Jianger, Children's Day aesthetic creative thick painting, Rich elements and unique style of retro creative illustrations, Flat illustrations with a summer atmosphere and realistic scenes, Vibrant and charming thin solid lines and comic style, Full of childlike round shapes, Full of childlike imaginative illustrations, American style full of childlike fun and rich details, Fun cartoon illustrations full of details and full pictures, Illustrations with soft contrast of light and shadow, Claude Monet, Cthulhu variant research organization base, The mysterious three pillars of Cthulhu mythology, Panoramic visual illustrations with delicate details and exquisite local pictures, Six or seven qualities, Orchid  chrysanthemum  plum and bamboo element patterns, Concrete and geometric animal tattoo patterns, Realistic approach to express abstraction, Nongfu Spring packaging illustrations, Lingyin's demon, Geometry, Fantasy symphony of geometry and color flattening, Geometric irregular vector graphics with large color blocks, Geometric picture line gradient color flat style coffee brand, Combination of geometric shapes and bright tones, Geometric conceptual illustration, Knife, Silhouette, Paper-cut collage composition is full of bright colors and gradients, Paper-cut art style, Seijima Seiki, Office modeling icon, Anime two-dimensional character gaku, Animal Crossing game screen, Anime series blue-eyed samurai screen exquisite, Bauhaus, Bauhaus Eton Dutch style school clear line painting style, Hungarian illustrator Susan Batori, Cosmetic girls' beauty and cartoon styling, Medical beauty illustrations, The twelve zodiac signs are personified  colorful and complex, The twelve zodiac signs illustration design Cangyuan Muxue, Sixteenth-century bookplate prints, Hua Sanchuan's flying dragons and phoenixes, Cartoon 1, Cartoon 2, Cartoon character design pencil manuscript, Cartoon hand-painted style with fine and smooth black and white graffiti, Cartoon vector Q version villain, Indian illustrator maiyakala, Indian culture and art symmetrical aesthetic patterns, Impressionism, Depressing dark horror with texture effect, Thick coating texture GUCCI commercial illustration, Original nature ethnic minority oriental art, Summer is a dream of Watermelon, Original painting 1, Original painting cyberpunk style science fiction elements, Original God commercial original illustration spring  summer  autumn and winter, Two-color woodcut print flower girl, Double exposure, Dystopia 1, Dystopia 2, Dystopia 3, The glowing girl is gentle and soft, Ancient magnificent national style picture book Lichengchengcheng, Classical and strange  gorgeous and magnificent decorative patterns, Classical paintings for modern reconstruction, Classical aesthetics and soft tones abstract style, Classical style and romantic temperament prints, Ancient Egypt, Ancient watercolor pen, Ancient style oriental aesthetics rock color four beauties series, Ancient style character illustration love story, Ancient style Hua Zhang Yi Pipa Xing details, Ancient style and ancient charm life scenes, Ancient style scene illustration Liao Zhai series, A world where cuteness and horror coexist, Cute healing warm illustrations with bright colors and smooth lines, Cute stories, Cute picture book style little girl with big eyes, Shi Zhifang's hand-painted Huizhou architectural works, Epic sci-fi structures and urban landscape futurism, Synthetic pictures of dazzling starry sky, Ghibli style, Post-Impressionism, Daidai Life uivi, Flat painting of Harvard Dunhuang Museum, Gothic, Gothic gloomy realism 2, Gothic fairy tale style, Gothic weird style playful girl doll, Gothic style stop motion animation box monster, Nezha: The Devil Child's Birth Concept Design, Thangka 3, Aesthetic healing illustrations of the beauty of the four seasons, Commercial original illustrations XXXuAn, Commercial illustrations 1, Commercial illustrations 11, Commercial illustrations 2, Commercial illustrations 3, Commercial illustrations 4, Commercial illustrations 5, Commercial illustrations 8, Commercial illustrations Tustin series, Commercial illustrations of the rising and setting moon, Commercial illustrations of flowing lines with just the right amount of noise, National treasures of cultural relics anthropomorphic series illustrations, National treasures of exquisite posters, National trend elements of commercial illustrations of national charm of provinces series, Guochao board painting rock color ancient style Chinese elements ancient stories, Guochao style, Chinese painting ink painting Ma Qibi, Chinese painting comic strip painted white-haired girl, A fantasy journey of the Forbidden City combining Chinese style and childlike fun, Chinese style illustration night rain sent to the north a painting and a poem ready to come out, Chinese style illustration cicada chirping, Chinese style painter Xijiu xj's work candle and dream painting collection, Schematic portrait style, Pattern and decorative movement, Pattern decorative style arts and crafts, Chart drawing style, Changing between brilliant growth and cruel death, Complex scene perspective  retro and childlike cartoon, Basic shape splicing, Tarot card character design, Zelda: Breath of the Wild, Coloring book, Ink line drawing 1, Ink line drawing 4, Spectacular grand luminous scene CG, Retro rich colors  magnificent trendy portrait illustration, Retro two-dimensional comic style, Retro collage element creation painting, Retro digital art illustration Chinese flowers and birds blue print, Retro fashion lines interpret timeless elegance, Retro Showa illustration style, Retro futuristic utopian illustration works, Retro European lines with complex and delicate Art Nouveau style, Retro romance full of artistic decorative elements, Retro aesthetic patterns and stunning art, Retro color matching character outfit creative illustration, Retro color illustration style city poster, Retro color matching home aesthetic mathematical drawing, Retro rust red flat style illustration, Retro style illustration color matching harmonious details density contrast, Retro style architectural scene modeling concept design, Retro style illustration cat's elegant life, Complex graphics and rich details mechanical style cartoon illustration, Alien icon uivi1, Alien icon uivi2, Alien icon uivi3, Retro style illustration full of technology in the multiverse, A gorgeous and beautiful world with multiple colors overlapping, Multi-dimensional surrealism style purely detaches the sensory body, Large silhouette set scenery illustration, David Hockney's bold use of colors with strong contrast, David Hockney's love for real life, Large stainless steel animal sculptures are also crazy about scrap iron, Large brushstrokes render a strong sense of volume concept original painting, Bold and bright colors with a strong visual sense of flat style illustration, Creative illustration of urban children in garlic, Large perspective composition with cold tones and a sense of technology, Large perspective special light graffiti style American illustration, dalong animal scene, Angel hunting area Japanese retro, Exaggerated figure limbs and generalized pictures, Exaggerated Gothic fantasy European and American illustrations, Exaggerated shapes and straight lines, Exaggerated figures and plants, Exaggerated human proportions plus elements and colors in a spectral style, Wonderful unorganized themes and chaotic compositions, Fantasy retro atmosphere and soft color scene illustrations, Fantasy colors and bizarre oriental world, Illustrator with wonderful ideas and innocence, Female Concerto Series Prints Chen Boqing, Nana sauce Yoshi vector pattern, Memphis style, Memphis colorful and interesting illustrations, Seasonal changes C4D scene illustrations with a sense of story, The bizarre world of a lonely star, Tranquility is like a beautiful poem in daily life, Stop-motion animation Year of the Rabbit, Experimental art future geometric vision, Interior Design 1, Interior Design 2, Interior Design 3, Hayao Miyazaki style, Three-dimensional 3D paper sculpture, Fable story and famous book illustration woodcut, Searching for the traditional pastry series illustrations in Jiangnan, Focus on the artist's paintings, Little Rabbit and Mr. Wolf Cute Healing and Warm Picture Book, Xiao Linfan's Galaxy Print Beautiful, The combination of daily life and fantasy of kittens, Xiaohualang Retro Skateboard Pattern Design, , Existing Patterns, Local Anatomy 1, Local Anatomy 2, Local Anatomy 3, Mountain and Sea Punk Style Illustration, Yamada Akihiro, Lingnan School of Painting 1, Lingnan School of Painting 2, Kawamata Satoshi Japanese Painting Rock Color, Kawase Misui Architectural Landscape Painting, Industrial Original Painting, Industrial Style, Detailed and Colorful Comic Strip of Trouble in Heaven, Crafts, Use lighting to create atmosphere and environment concept painting, Baroque period, Blanche's science fiction illustrations  mechanical traces of the old times, Common people's food and Chinese style, Greek mythology story Hawthorne 1922, Clean and neat color block scene illustration, Clean  modern and advanced illustration graphics and layering, Flat light scene detailed depiction of objects, Ordinary scene synthesis movie poster brain hole, Heisei aestheticism Japanese Ukiyo-e, Fantasy temple and crowd, Humorous style and exquisite painting skills comics, Modeling 1, Modeling 2, Modeling Game of Thrones Online, Modeling the Hut, Architectural Sketch 1, Architectural Sketch 2, Starting a Magical Journey at Night, Strong contrast  delicate lines  misty and gradually changing  moist emotions, Strong and rich colors  rich brushstrokes  lines and shapes, Strong light and dark contrast game card design, Strong color contrast expresses the inner world, Strong black and white contrast and movement moments, Contemporary fine brushwork painting is gorgeous  romantic and elegant, Metaphysical style, Colored comic strip Goddess of the Luo River, Stained glass window 1, Colored pencil hand-painted transparent fragile picture gentle, Colored pencil illustration color emotional aesthetics, Slightly fluorescent color illustration, Miniature movie style, Sibo Palace Museum scarf pattern, Grotesque and playful sense of colorful colors 3D rendering, Grotesque and humorous flat painting illustration, Valentine's Day theme flat illustration love gift, Valentine's Day theme illustration, Emotional flower language illustration series, Amazing at the use of pen lines, Fright Town Stop Motion Animation, Feel the romance of spring  colorful and dreamy, Gordon Mortensen's out-of-print woodcut landscape, Flat geometric lines and color blocks express passion and pursuit, Flat animal style illustrations with smooth lines and retro tones, Flat design tones tend to be cartoon funny girls, Flat cute small illustrations with handmade textures, Flat color block painting rough texture, Flat style character illustrations with high saturation colors, Flat style animal illustrations with healing elements, Flat style illustrations with life community, Flat style, Flat style texture light novel illustrations, Handmade clay modeling magic potion, Hand-painted style, Hand-painted style black and white manuscripts with charming lines, Hand-painted style with delicate and complex black and white graffiti tends to be realistic, Turn famous paintings into 8bitAdamLister, Melting the dust of stars into rock color, Abstract watercolor architectural street scene Viktoria, Abstract 1, Abstract 2, Abstract Expressionism, Abstract Expressionism 1, Abstract surreal psychedelic gorgeous colors 3D and 2D combination, Ramen theme retro illustration poster Ukiyo-e color matching, Byzantine style 1, Byzantine style 2, Life on the palm Koi commercial illustration, Illustration poster, Watercolor works that are good at capturing the subtle essence of shadows and various light and shadows, Dunhuang Zodiac Series National Trend Style Cultural and Creative VI Design, Dunhuang Auspicious Retro Elements Illustration, Renaissance, Renaissance Woodcut, Zebra Western Town, Mottled and dazzling picture style full of free imagination, Slovak Folk Tales Buried Sword Picture Book, New Chinese National Style Dream Brush Flowers Water Mirror Clouds and Sky, New Chinese Style, New Classical Pastoral Flowers and Birds Background Wall Decoration, New National Style Chinese Elements Flat Texture Line, Sinkai Makoto, Art Nouveau, Neo-Decorative Style Geometric Flatness, Silent Dreams  Gorgeous Colors  Flexible and Light Brushstrokes  and Uplifting Composition, Daylight Printing, Interesting Illustrations of Daily Life, Japanese Style God and Demon Style Illustrator Kou, Japanese Fresh Style 1, Japanese Fresh Style 2, Japanese Cut Painting  Large Hollow Design  Exquisite Paper Sculpture, Japanese Animation, Japanese Graphic Design Poster Style 1, Japanese Graphic Design Poster Style 5, Japanese Ukiyo-e Combined with Modern Elements  Delicate and Unrestrained Wonderful Magic, Japanese Ukiyo-e Style 1, Japanese Ukiyo-e style 2, Japanese manga style, Japanese artist black fairy tale style flat painting, Early Rice, Fashion character collage 1, Fashion character collage 2, Fashion business flat style illustration parent-child camping mall music, Fashion girl silhouette summary, Fashion illustration lines are simple and clean, Bright colors  grand scenes  dreamlike pictures, Landscape illustrations on postcards, Chiaroscuro painting method 1, Bright healing architectural illustrations, Dark Gothic style, Watercolor illustrations of dark Gothic and French Rococo, Dark pop surreal and bizarre fairy tales, Flat illustrations of Muli low-alcohol wine packaging design with fresh colors, Moon River simple illustrations surreal, Wooden Bottle Brand Casting Bureau Trendy Vector Illustrations, Woodcut retro style picture book illustrations with natural and fresh tones, Woodcut prints are rough and magnificent  but full of struggles and entanglements, Woodcut prints in black and white Stokes wonder book, The clever treatment of black and white in woodcut prints creates different rhythms and rhymes, Woodcut 2, Woodcut 3, Woodcut 4, Simple ethnic elements and wild imagination, Mechanical advanced fashion photography, Relaxed lines and soft retro colors, The extremely tense and dynamic figures and the abstract geometric background create a strong but harmonious contrast, Highly appealing black and white illustrations, Minimalism, Minimal lines are cute and healing illustrations are colorful, Minimal sports venues and light and shadow, Maximalism, Maximalism Temple Series, Maximalism seeks for beauty without form, Maximalism is rich in color and detailed illustrations, Maximal illustrations are delicate and rich in details and healing, Maximal illustrations are colorful and delicate scenes, Extreme black and white original illustrations Lithuania Rokas, Constructivism and Cubism style geometric shapes beauty straight lines and curves to form the outline, Soft picture quality strong light and shadow blue tone, Soft color system combined with block brush material, Soft colors and exotic patterns Wuyang Yu, Bridge book version of the six guys left in the shoe beautiful illustrations, Dream Wall Cthulhu Mythos Xumi, Dream fantasy feeling post-filter, DreamWorks style, Dream colors beautiful painting style imaginary world, Dream laser style, Van Gogh, Diary of a Forest Girl, A peaceful and leisurely life in the depths of the forest, Forest style, Conceptual original painting design Wizards of the Coast, Concept scene original painting black and white draft, Concept Art 1, Concept Art 2, Concept Art 3, Concept art original painting Horizon West: Despair, Concept art design original painting Thomas, Concept art style, Concept design exquisite scene endless imagination, Simulated photo 2, Simulated photo 3, Op style, European and American style watercolor large color block life rough, European and American style color block portrait, Absolute color sense dimension fantasy that deceives the eye, Picasso Blue Period, National Characteristic Art 1, National Aesthetics Figure Illustration Design, National Style, Folk Art Geometric Abstractionism, Bubble 3D, Watermark Woodcut West Chamber, Ink and Wash Chinese Style Hermit Fantasy, Ink and Wash Illustration, Ink and Wash Painting Ancient Style Animal Anthropomorphism Series, Ink and Wash Painting Lines Freely Vertical and Naturally Blurred, Ink and Wash Painting Comic Strip West Lake Main Ink is Rough but Not Delicate, Ink and Wash Painting Style is Elegant  Elegant and Thick, The Fusion and Collision of Ink and Wash Aesthetics and Trendy Culture, Ink and Wash Style, Ink and Wash Style Blurred Mountain Ghost Series, Watercolor Master Joseph's City Walk, Watercolor illustration of the fairyland on the other side of the dream, Watercolor healing notes from nature, Watercolor 4, Watercolor keeps the color rich and flat, Watercolor is fresh and elegant  exquisite and small, Watercolor flower soul series ancient Chinese elements, Watercolor blue dream, Watercolor style impressionist dotted strokes, Watercolor pen drawing 3, Watercolor style freehand painting Zhang Zhaofang, Watercolor style and texture Russian fairy tale illustration, Watercolor style color retro animals and plants, Watercolor style landscape free and love, Crystal animal modeling, Murals of the Sanqing Hall of the Yongle Palace, Hiroshi Nagai, Two-dimensional comics with the sense of déjà vu of samurai in the Edo period, Oil painting 1, Oil painting 2, Oil painting 3, The quiet and silent power of colors in the oil painting world, Oil painting healing scenery walks into the bright spring, Oil painting color texture unique painting, Oil painting texture life freehand illustration, Oil painting style single color detailed detail portrayal, Healing and comfortable pixel style daily life, Healing romantic illustrations warm and cute, French post-impressionist Paul Ranson, French Art, French Symbolist Paintings Blue Sorrow and Noise, Pop Art, Focus on the treatment of the volume of the object Orderly sense of space, Rococo, Pattern Japanese elements Urban trend Creative illustration, Flowing lines Noise sense Fashion illustration, Smooth and soft lines Strong color contrast, Thick oil painting 1, Thick oil painting 2, Thick oil painting 3, Thick ink grooves and heavy colors are used to render the high-spirited youth in the brush and ink, Intense colors and rich details Museum oil painting, The strong traditional ink painting style shows the world of monsters, Rich colors plus rough brushstrokes, Rich colors  mysterious atmosphere  unique brushstrokes, Raccoon fish building scene, Romantic rich details full of yellow balloon picture book, Romanticism, Romantic gentle tones realistic fantasy, Life is like a dream  feathered into a fairy  watercolor painting of clouds and ghosts, Poster material Mid-Autumn stereoscopic vision, Marine ecology marker pen hand-painted, Marine style, Graffiti, Graffiti cartoon style complex lines retro tones, Mixed silhouette animal illustration series, Fresh flat painting illustration, Fresh graffiti illustration, Gradient illustration style, Warm textured shapes and bold colors to weave atmospheric stories, Warm color blocks flat painted eyes, Warm children's insert, Warm healing people and nature, Warm life icon uivi, Warm fairy tale picture book colorful nature, Game scene picture 1, Game scene picture 2, Game style 1, Game style 2, Xiangye walking corpse, Wet plate photo, Beautiful three-dimensional paper art, Comics, The combination of lighting and composition is like a screenshot from a movie, Pointillism, Photo-level realism, Alice in Wonderland theme illustration background reveals the special texture of the letters, Printmaking, Pencil draft of characters on kraft paper, Unique style hand-painted style girl illustration, Unique and amazing color matching is refreshing and healing, Glory of the King original painting is gorgeous  delicate and unique in details, Environmentally friendly and fresh, Modern, Modern luxury style, Modernism, Modern minimalist style, A colorful world combining reality and fantasy  joyful and lively, Realistic watercolor painting of simple and real life fragments, Pearl milk tea style, Happy Halloween  Brother Yao, Life scene perspective architecture healing color illustration, Life scene sketch full of details, Use geometry to build the world, Use gorgeous dark skull art to contain racial discrimination issues, The American painting style with rich and bright colors is very individual, The bold and gorgeous colors are cleverly composed with warmth and energy, Use colors to explore the explosive emotions when people try to deconstruct themselves, Film photography style, Film screen 1, Rich  delicate and exquisite pictures with harmonious color matching healing illustration, The illustrator whose pictures are always full of mystery, Illustrations with leisure and childlike fun, Flat painting illustrations with no more than four colors, Delicate and exquisite black and white decorative illustrations with needle-shaped pens, Cute style  smooth and round lines  comics, Innocent and dreamy style  clear texture  illustrations, Simple and clean style  warm and healing picture books, Simple and fresh style  rich and delicate details, The delicate style is in the picturesque water town  enjoying the prosperity of the world, Illustrations of plants and animals summarized by color blocks with a slight sense of volume, Mrs. White Rabbit Picture Book, White Art Miracle Thick Painting, White Visual Reality Engine, White Goose Girl Pure Ethereal Composition Fantasy Color, Changeable, Picture Book Story Hundred Years Ago, Hundred Years Old Picture Book The children's corner1915, Pixar Animation Style, Shadow Art and Details, Shadow Style, Hanfu Commercial National Trend Illustrations in the Prosperous Tang Dynasty, Combination of Real Objects and Illustration Elements, Real, Vector Graphics 3, Vector Three-Dimensional Urban Illustrations, Vector Style Illustrations Technology and Life Full of Details, Mineral Heavy Color Painting Spring Breeze Flowers and Grass Fragrance Fan Shu, Hard-core National Trend Concept Illustrations, Mysterious color matching with strong decorative effect, Seed painting, Tanemura Arina's old Japanese comic style, Science fiction woodcut comic character elements, Science fiction color lines and fine two-dimensional comics, Science fiction style metal cold sweet taste, Qinqiang opera non-legacy long scroll national trend cultural and creative design, Ethereal and vague fascinating profound charm, Cubism, Fairy tale picture book Seven Crows pencil graphite digital, Fairy tale picture book style, Fairy tale style, Childlike cute cartoon illustrations with simple lines, Strong brushstrokes  high-purity colors  rich light and shadow  scenes depicting fantastic and magnificent colors, Exquisite brushstrokes  warm and unique color matching, Exquisite brushstrokes  colorful cartoon element illustrations, Brushstrokes  color blocks  splicing  stacking  bold use of colors, Wait until I grow up a little more children's picture book, Isometric anime style, Isometric art style, Simplified characters narrate the social conditions in the self, Simple but beautiful  lonely and profound, Simple and interesting line style  unique and expressive illustrations, Simple line flat painting  bright colors  use black to pinch key points cartoon painting, Simple line pencil drawing  childlike style graffiti, Simple and bold contrasting colors  flat logo, Simple and fashionable same color, Simple life illustration, Simple and advanced natural aromatherapy packaging design, Simple blue office illustration, Similar to jelly pie vortex spiral composition dreamy and romantic, Pink lines freehand Chinese light and soft dream, Pink and blue color matching delicate line drawing sweet style, Roughism, Rough large perspective black and white line drawing, Rough charcoal sketch 1, Rough line flat color Disney related, Exquisite and delicate line Thumbelina illustration, Exquisite and cute noise illustration glass feeling, Exquisite and delicate appreciation of the stunning garden, Exquisite and mysterious black and white universe, Sketch hand-painted style black and white details, Sketch style realism detailed portrayal, Sketch style hand-painted style black and white world, Sketch black and white gray ethereal and weird feeling, Prosperous and glorious gathering place, Under the prosperous city illustration poster black and white texture, Extremely complex local magnification has very large elements and content worth savoring, Complex and gorgeous colors and complex composition have great visual impact, Dream of Red Mansions Liu Dan's house painting, Red and black fantasy illustration works, Pure graphics  lines and colors are harmonious, Paper color ink 1, Paper Color Ink 2, Texture Retro Tone Less is More Creative Concept, Line Drawing Illustration Same Color Noise Gradient, Line Drawing Healing Fashion Landscape, Smooth Lines Bright Colors Complex Composition Commercial Illustration Details, Smooth Lines Fresh Colors Violin Song, Ink painting with dense and sparse lines and strong black and white contrast, Simple and soft lines  unique composition and perspective  and wonderful light and shadow effects, City and natural landscape illustrations with casual lines, Casual lines and concise pictures, Thin lines with shadows and low saturation illustrations, Delicate and elegant fantasy sculptures with vivid shapes, Delicate and smooth brushstrokes and clever color matching tell the story of Zhong Kui catching ghosts, Beautiful paintings with delicate colored pencils full of fantasy colors, Delicate brushstrokes describe warm and lively pictures, Delicate paper art works, Delicate lines and dark tones convey the fragility of human nature, Exquisite lines  gentle colors  and beautiful painting style, Exquisite lines  black and white animal decoration paintings, Exquisite and casual lines  extremely exquisite and gorgeous details, Details depict rich illustrations of a corner of the city, Detail control ecstasy  one car  one city  one life, Cartoon illustrations full of details and fun, Combining dots  lines  shadows and other textures to depict a fairy-tale world, Quilting art, Reading ancient poems and learning Chinese characters in picture books, Victorian era, Romantic weddings in the Victorian era accompanied by floral fragrance and poetry, Green and magenta picture book screen, Colorful fruit characters  exaggerated flat illustrations with bright colors, Luo Ci Q version Gothic two-dimensional vision, Yang Yang Super Energy Baking House Rough Texture Stop Motion Animation, American Golden Age Retro Commercial Illustrations with Tough Brushstrokes, American Country Style, American Cartoon Illustration Style, American Retro Marvel Realism, American Retro Comics, American Retro Comics Science Fiction Elements, American Retro Trend Illustration with Hands as the Main Element, American Life Illustration, American Style Oil Painting 2, American Black and White Cartoon Character Illustration, American Comics Rough Realistic Style Street, American Comics Style Lines are Delicate and Full of Details, Food House, Ultramarine, The Old Man and the Sea Illustrations Knife Marks Engraving Prints, Old Old Fish Children's Literature Beautiful Paintings Warm and Fresh Colors, Liao Zhai Nie Xiaoqian Picture Book Artistic Conception, Texture Illustration Style, Hu Yefo's Fine Brushwork Ladies with Charming Emotions, Paying Tribute to Classic Movies Pixel Style, Color Block Flat Painting Architecture Nature, Colorful and Vivid Imagination Art Illustrations, Color and Fun are the Antidote for Healing, Harmonious Color Matching Rich Layers Full of Details, Bright Colors Warm and Healing Illustrations, Beautiful Colors Harmonious Pictures Mature and Rendering Power, The colors are warm and full  the pictures are complicated and luxurious, The colors are numerous but not messy  the soft tones and light and shadow processing are matched with warm colors of similar colors, The colors are saturated and rich  the composition is varied and has visual tension, The small scene illustrations with low color saturation combine beverage packaging with architecture, The iconic buildings of various countries are vivid in color, The colorful and eye-catching daily necessities illustrations, The colors are elegant and the brushstrokes are delicate and creative illustrations, The daydream of an art urchin, Elden fanfiction European and American style, Floral flat illustration 1, Floral flat illustration 2, Floral flat illustration 3, Bud people Tu Tu, Prairie style, Yayoi Kusama, Yayoi Kusama day36, Fluorescent color palette, Dutch De Stijl, Mobius Final Fantasy, Mondrian, Steampunk, Vaporwave 2, Vaporwave style BerlinMichelleart, Vaporwave style with polka dot elements, Blue ballpoint pen drawing, Blue fantasy dazzling colors and visual effects, Blue flat style illustration, Blue fine texture stacking, Scene dominated by blue and yellow tones, Rainbow painting 1, Ant 1, Ant 2, Crayon painting 1, Crayon painting 2, Crayon painting 3, Walking in art, Street culture elements are colorful, Street pop art and three-dimensional art vector geometric graphics, Street graffiti elements urban culture fantasy classical art, Expressionism, Expressionism 1, Expressionism 2, The frozen moment of light and shadow watercolor hand-painted, Xiyue Wonder Child stop-motion animation, Western painting combined with Japanese art classics and decorativeism, Journey to the West: Havoc in Heaven feels the charm of the classics, Character modeling is cute and adorable 3D modeling, Analysis style, Textbook illustration style concise lines render the noble and elegant temperament of the characters, Real texture and transparent elements with diverse shapes and full of imagination, Trendy art combining cyberpunk and dystopia, Cyberpunk and mecha style colorful fantasy visual performance, Cyberpunk scene original painting concept design, Cyberpunk style illustration gang poster, Hyperrealism, Hyperrealistic retro optical illusion, Surrealistic composition illustration NiNE Xiaojiu, Surrealistic pop style Japanese cultural elements, Surrealistic painting with delicate brushstrokes and light retro tones, Surrealistic retro art 1, Surreal Retro Art 2, Surreal Retro Art 3, Superb scene space sense horror aesthetics, Vietnamese rural illustrations in spring rainy season, Zichu ethnic patterns that can't catch up with the popularity, Manic technical pen drawing bold and gorgeous color matching, Light retro decorative painting simple atmosphere, Easy and warm illustration low brightness high saturation, Light neon style fresh healing illustration, Dali, Daguerreotype, Comic strip Daiyu burying flowers with delicate and beautiful brushwork, Disney style 2, Charming abstract art fantasy painting world, The labyrinth illustration is rich in details and bright in color, Psychedelic punk style concept original painting design, Psychedelic futuristic space opera, The psychedelic atmosphere and unique composition, Camouflage dream photo filter, Express the theme through the combination of color graphics and background, Modeling clay 2, Modeling clay 3, Painting is made by using the carving knife to convey emotions  color woodcut, Stamp illustration style 1, Stamp illustration style 2, City, City beauty pink nightlife, Retro color matching and soft composition  symmetrical and repeated geometric elements  rhythmic sense, Strong color matching  gorgeous details  and classical beauty, Acidic style, Revisiting the warmth and beauty of the Little Prince  this fairy tale is not for everyone, Fauvism 1, Wild Dogs and Richness, Metallic Acid Element 1, Metallic Acid Material Elements, Metallic Acid Material Modeling and Rendering, Gold and Dark Collision  Epic Painting, Pinhole Photo 1, Pinhole Photo 2, Hand-painted with a needle pen  complex line drawings  strong yellow marker style, Pen Illustration 1, Pen Illustration 3, Pencil Sketch 1, Pencil Sketch 4, Silver Li Pattern Animals, Intricate and rich pictures are very bright large scene illustrations, Well-arranged collages, Laser style fantasy colors are beautiful and bright  and the atmosphere is full, Epidemic prevention propaganda stay at home and pay attention to safety 3D rendering, Gloomy and heavy style and surging emotions, Onmyoji mobile game Shikigami, Afanti's story stop-motion animation, Chen Ke's Bauhaus Girl Series, Reading Shanhaijing picture books with children, Ceramic art national characteristics alternative world, The fairy tale of the dark temperament of ceramics, The casual and strong colors are soft and simple  and the picture is full of passion and emotion, The random lines and gradient colors form a magical illustration, Engraving illustration 2, Engraving illustration 3, Engraving print 1, Engraving print 2, Engraving art style 1, Engraving art style 2, City in the rain, Neon color two-dimensional illustration, Neon city futuristic vapor wave, Pili puppet show stop motion animation, Green landscape painting Xue Liang's image landscape, Blue Printing Method 1, Blue Printing Method 2, Still Life Oil Painting Dreamlike Still Life Painting, Exquisite Ancient Style Painting of Intangible Cultural Heritage Anthropomorphic Series, Scene Illustrations by Korean Illustrator Won Jun Tae, Specially Rendered Blurred Illustrations by Korean Illustrators, Korean Cartoonist JaeKwang Park, Korean Painter's Silent and Warm Universe, Bright and Colorful Colors  Cute and Cute Illustrations, Fresh Colors  Dark Gray  Proper Stroke Density, Colorful Colors  Strong Contrast of Light and Dark  Increases Visual Impact, Bright  Lively and Rich Style  Fantastic Ideas  Create a Colorful and Smart Illustration Universe, Unique style commercial illustration with exquisite and smooth lines, Unique style black and white illustration, The style is gloomy and strong  using small areas of high saturation contrasting colors to render the mood of the picture, The cloth bag of the wind god, Mosaic painting, Bone corn rice thickly painted Korean style, High saturation color music theme illustration poster, Ghost clan thunder god legend super cute stop motion animation, Magic color illustration, Fishing fairy grocery store looking for abstraction, Bright and vibrant colors are fresh and cute, Bright colors and quirky style original illustration, Yellow light sword, Dark micro-flavor illustration, Black and White, Black and White Book Pencil Drawing, Black and White Leisure and Simple Life Scene Illustration, Black and White Office Illustration, Black and White Fine Brushwork and Line Drawing National Trend Elements Chinese Charm Illustration, Black and White Illustration Full of Childishness and Exquisite Pictures, Black and White Illustration Brushstrokes are Vigorous and Delicate, Black and White Illustration Lines are Tough and Weird, Black and White Illustration of Children Following the Bagpiper, Black and White Polka Dot Line and Surface Illustration, Black and White Decorative Painting Leshan Giant Buddha, Black and White Marker Pen Textured Weird Illustration, Black and Gold Terrorist Style, Qiwu Art Exhibition Poster and Extension Design, 

==> sec/2_formatting.tex <==
\section{Formatting your paper}
\label{sec:formatting}

All text must be in a two-column format.
The total allowable size of the text area is $6\frac78$ inches (17.46 cm) wide by $8\frac78$ inches (22.54 cm) high.
Columns are to be $3\frac14$ inches (8.25 cm) wide, with a $\frac{5}{16}$ inch (0.8 cm) space between them.
The main title (on the first page) should begin 1 inch (2.54 cm) from the top edge of the page.
The second and following pages should begin 1 inch (2.54 cm) from the top edge.
On all pages, the bottom margin should be $1\frac{1}{8}$ inches (2.86 cm) from the bottom edge of the page for $8.5 \times 11$-inch paper;
for A4 paper, approximately $1\frac{5}{8}$ inches (4.13 cm) from the bottom edge of the
page.

%-------------------------------------------------------------------------
\subsection{Margins and page numbering}

All printed material, including text, illustrations, and charts, must be kept
within a print area $6\frac{7}{8}$ inches (17.46 cm) wide by $8\frac{7}{8}$ inches (22.54 cm)
high.
%
Page numbers should be in the footer, centered and $\frac{3}{4}$ inches from the bottom of the page.
The review version should have page numbers, yet the final version submitted as camera ready should not show any page numbers.
The \LaTeX\ template takes care of this when used properly.



%-------------------------------------------------------------------------
\subsection{Type style and fonts}

Wherever Times is specified, Times Roman may also be used.
If neither is available on your word processor, please use the font closest in
appearance to Times to which you have access.

MAIN TITLE.
Center the title $1\frac{3}{8}$ inches (3.49 cm) from the top edge of the first page.
The title should be in Times 14-point, boldface type.
Capitalize the first letter of nouns, pronouns, verbs, adjectives, and adverbs;
do not capitalize articles, coordinate conjunctions, or prepositions (unless the title begins with such a word).
Leave two blank lines after the title.

AUTHOR NAME(s) and AFFILIATION(s) are to be centered beneath the title
and printed in Times 12-point, non-boldface type.
This information is to be followed by two blank lines.

The ABSTRACT and MAIN TEXT are to be in a two-column format.

MAIN TEXT.
Type main text in 10-point Times, single-spaced.
Do NOT use double-spacing.
All paragraphs should be indented 1 pica (approx.~$\frac{1}{6}$ inch or 0.422 cm).
Make sure your text is fully justified---that is, flush left and flush right.
Please do not place any additional blank lines between paragraphs.

Figure and table captions should be 9-point Roman type as in \cref{fig:onecol,fig:short}.
Short captions should be centred.

\noindent Callouts should be 9-point Helvetica, non-boldface type.
Initially capitalize only the first word of section titles and first-, second-, and third-order headings.

FIRST-ORDER HEADINGS.
(For example, {\large \bf 1. Introduction}) should be Times 12-point boldface, initially capitalized, flush left, with one blank line before, and one blank line after.

SECOND-ORDER HEADINGS.
(For example, { \bf 1.1. Database elements}) should be Times 11-point boldface, initially capitalized, flush left, with one blank line before, and one after.
If you require a third-order heading (we discourage it), use 10-point Times, boldface, initially capitalized, flush left, preceded by one blank line, followed by a period and your text on the same line.

%-------------------------------------------------------------------------
\subsection{Footnotes}

Please use footnotes\footnote{This is what a footnote looks like.
It often distracts the reader from the main flow of the argument.} sparingly.
Indeed, try to avoid footnotes altogether and include necessary peripheral observations in the text (within parentheses, if you prefer, as in this sentence).
If you wish to use a footnote, place it at the bottom of the column on the page on which it is referenced.
Use Times 8-point type, single-spaced.


%-------------------------------------------------------------------------
\subsection{Cross-references}

For the benefit of author(s) and readers, please use the
{\small\begin{verbatim}
  \cref{...}
\end{verbatim}}  command for cross-referencing to figures, tables, equations, or sections.
This will automatically insert the appropriate label alongside the cross-reference as in this example:
\begin{quotation}
  To see how our method outperforms previous work, please see \cref{fig:onecol} and \cref{tab:example}.
  It is also possible to refer to multiple targets as once, \eg~to \cref{fig:onecol,fig:short-a}.
  You may also return to \cref{sec:formatting} or look at \cref{eq:also-important}.
\end{quotation}
If you do not wish to abbreviate the label, for example at the beginning of the sentence, you can use the
{\small\begin{verbatim}
  \Cref{...}
\end{verbatim}}
command. Here is an example:
\begin{quotation}
  \Cref{fig:onecol} is also quite important.
\end{quotation}

%-------------------------------------------------------------------------
\subsection{References}

List and number all bibliographical references in 9-point Times, single-spaced, at the end of your paper.
When referenced in the text, enclose the citation number in square brackets, for
example~\cite{Authors14}.
Where appropriate, include page numbers and the name(s) of editors of referenced books.
When you cite multiple papers at once, please make sure that you cite them in numerical order like this \cite{Alpher02,Alpher03,Alpher05,Authors14b,Authors14}.
If you use the template as advised, this will be taken care of automatically.

\begin{table}
  \centering
  \begin{tabular}{@{}lc@{}}
    \toprule
    Method & Frobnability \\
    \midrule
    Theirs & Frumpy \\
    Yours & Frobbly \\
    Ours & Makes one's heart Frob\\
    \bottomrule
  \end{tabular}
  \caption{Results.   Ours is better.}
  \label{tab:example}
\end{table}

%-------------------------------------------------------------------------
\subsection{Illustrations, graphs, and photographs}

All graphics should be centered.
In \LaTeX, avoid using the \texttt{center} environment for this purpose, as this adds potentially unwanted whitespace.
Instead use
{\small\begin{verbatim}
  \centering
\end{verbatim}}
at the beginning of your figure.
Please ensure that any point you wish to make is resolvable in a printed copy of the paper.
Resize fonts in figures to match the font in the body text, and choose line widths that render effectively in print.
Readers (and reviewers), even of an electronic copy, may choose to print your paper in order to read it.
You cannot insist that they do otherwise, and therefore must not assume that they can zoom in to see tiny details on a graphic.

When placing figures in \LaTeX, it's almost always best to use \verb+\includegraphics+, and to specify the figure width as a multiple of the line width as in the example below
{\small\begin{verbatim}
   \usepackage{graphicx} ...
   \includegraphics[width=0.8\linewidth]
                   {myfile.pdf}
\end{verbatim}
}


%-------------------------------------------------------------------------
\subsection{Color}

Please refer to the author guidelines on the \confName\ \confYear\ web page for a discussion of the use of color in your document.

If you use color in your plots, please keep in mind that a significant subset of reviewers and readers may have a color vision deficiency; red-green blindness is the most frequent kind.
Hence avoid relying only on color as the discriminative feature in plots (such as red \vs green lines), but add a second discriminative feature to ease disambiguation.

==> sec/3_finalcopy.tex <==
\section{Final copy}

You must include your signed IEEE copyright release form when you submit your finished paper.
We MUST have this form before your paper can be published in the proceedings.

Please direct any questions to the production editor in charge of these proceedings at the IEEE Computer Society Press:
\url{https://www.computer.org/about/contact}.
